Federated Learning for Collaborative Inference Systems: The Case of Early Exit Networks

As Internet of Things (IoT) technology advances, end devices like sensors and smartphones are progressively equipped with AI models tailored to their local memory and computational constraints. Local inference reduces communication costs and latency; however, these smaller models typically underperform compared to more sophisticated models deployed on edge servers or in the cloud. Cooperative Inference Systems (CISs) address this performance trade-off by enabling smaller devices to offload part of their inference tasks to more capable devices. These systems often deploy hierarchical models that share numerous parameters, exemplified by Deep Neural Networks (DNNs) that utilize strategies like early exits or ordered dropout. In such instances, Federated Learning (FL) may be employed to jointly train the models within a CIS. Yet, traditional training methods have overlooked the operational dynamics of CISs during inference, particularly the potential high heterogeneity in serving rates across clients. To address this gap, we propose a novel FL approach designed explicitly for use in CISs that accounts for these variations in serving rates. Our framework not only offers rigorous theoretical guarantees, but also surpasses state-of-the-art (SOTA) training algorithms for CISs, especially in scenarios where inference request rates or data availability are uneven among clients.

==> math_commands.tex <==
%\usepackage[fleqn]{amsmath}
\usepackage{amsmath,amsfonts,bm,amssymb,dsfont}
\usepackage{array}
\newcolumntype{C}[1]{>{\raggedright\arraybackslash}p{#1}}
% \newcommand{\algorithmiccomment}[1]{\footnotesize{\textcolor{blue}{\hfill$\triangleright$~\footnotesize{\texttt{#1}}}}}
%\renewcommand{\mathbf}[1]{{\text {\bf #1}}}
\def\backbone{\pmb{\theta}}
\def\exit{\pmb{\phi}}
\def\inputx{\pmb{x}}
\def\output{\pmb{y}}
\def\prediction{\hat{\pmb{y}}}
\def\dataset{{\mathcal{D}}}
\def\receivedataset{{\tilde \dataset}}
\def\servedataset{{\hat \dataset}}
\def\servedatasetclient{\dataset^{s}_i}
\def\validdataset{\mathcal{V}}
\def\traindataset{\mathcal{T}}
\def\transdataset{\mathcal{TR}}
\def\numexits{{E}}
\def\lossfunction{L}
\def\E{\mathbb{E}}
\def\requestrate{\lambda^{g}}
\def\maxtransrate{\mu^{\mathrm{max}}}
\def\transrate{\lambda^{t}}
\def\fraction{f}
\def\optimprob{{\mathbb{P}}}
\def\weight{\alpha}
\def\approxloss{\lossfunction_{appro}}
\def\profile{\pmb{\lambda}}
\def\Profile{\Lambda}
\def\numlocalsteps{L}
\def\batch{\mathcal{B}}
\def\emploss{\lossfunction}%^{\mathrm{emp}}}
\def\genericfun{\mathcal{F}}
\def\lr{\eta}
\def\serverate{\lambda^s}
\def\numlevel{K}
\def\numnodes{n}
\def\serverateexit{\pmb{s}}
\def\setnodes{\mathcal{N}}
\def\setleafnodes{\mathcal{L}}
\def\setchildnodes{\setnodes^-}
\def\setparentnodes{\setnodes^+}
\def\setnodesexit{\mathcal{N}_e}
\def\model{\pmb{w}}
\def\N{\mathcal{N}}
\def\maxExit{E}
\def\reals{\mathbb{R}}
\def\naturals{\mathbb{N}}

\def\difficultySet{\mathcal{K}}
\def\setexits{\mathcal{E}}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\brackets}[1]{\left[#1\right]}
\newcommand{\parentheses}[1]{\left(#1\right)}
\newcommand{\card}[1]{\left|#1\right|}

\newcommand{\tremark}[1]{\textcolor{blue}{t: (#1)}}
\usepackage{mathtools}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\algrenewcommand\algorithmicrequire{\textbf{Input:}}
\algrenewcommand\algorithmicensure{\textbf{Output:}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

\newcommand{\old}[1]{\textcolor{red}{\cancel{#1}}}
\newcommand{\new}[1]{\textcolor{blue}{#1}}

%ADDED BY GIOVANNI 4/4/2024
\newtheorem{lemma}{Lemma}
\DeclareMathOperator{\VarVec}{{\mathbb{V}ar}}

\newcommand\scalar[2]{\langle #1, #2 \rangle}
\newcommand{\ww}{\boldsymbol{w}}
\newcommand{\vv}{\boldsymbol{v}}
\newcommand{\LL}{\boldsymbol{\Lambda}}
\newcommand{\LLa}{\boldsymbol{\tilde\Lambda}}   %weight used at aggregation
\newcommand{\wtce}{w_t^{(c,e)}} %not sure we will use this
\newcommand{\wtjce}{\ww_{t,j}^{(c,e)}} %model at client c when training exit e at round t and local step j
\newcommand{\Fce}{F_{c,e}}  %the empirical loss function at client c for exit e
\newcommand{\FSb}{F_{S,\LLa}} %the global empirical loss function targeted by our algorithm, potentially biased
\newcommand{\FSu}{F_{S,\LL\vphantom{\LLa}}} %the global empirical loss function we would like to target
\newcommand{\Fu}{F_{D,\vphantom{\LLa}\LL}}    %the actual goal
\newcommand{\Fb}{F_{D,\LLa}}    %the actual goal
\newcommand{\pce}{p_{c,e}} %the probability that that client c trains exit e
\newcommand{\Ce}{\mathcal C_e} %set of clients who are going to train exit e, i.e. those for which \pce>0
\newcommand{\Sep}{S_{e,\boldsymbol{p}}} %union of all datasets of clients who train exit e
\newcommand{\FSe}{F_{\Sep}}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\VC}{\textrm{VCdim}}
\newcommand{\Fe}{F_{D,e}} %expected loss at exit e
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\disc}{disc}
\DeclareMathOperator{\tv}{dist_{TV}}
\DeclareMathOperator{\Pd}{Pdim}
\DeclareMathOperator*{\argmin}{arg\,min}
%\DeclareMathOperator*{\Ex}{\mathbb{E}}
\DeclareMathOperator{\Var}{Var}
\DeclarePairedDelimiter\abs{\lvert}{\rvert}
%END ADDED BY GIOVANNI

